Similarity Problems in High Dimensions

The main contribution of this dissertation is the introduction of new or improved approximation algorithms and data structures for several similarity search problems. We examine the furthest neighbor query, the annulus query, distance sensitive membership, nearest neighbor preserving embeddings and set similarity queries in the large-scale, high-dimensional setting.

==> dmq/avg_upper.tex <==
\subsection{Average error}
\begin{theorem}
\label{thm:upperbound}

A $(r>0,c>0,\epsilon>0)$-distance-sensitive approximate membership filter with guarantees on the average error requires space:

\begin{align}
\BO{n\Big(\log\big(d\big)+\log\big(\frac{1}{\epsilon}\big) \Big)}&\text{ when } r<\sqrt{d/2}\\
\BO{n\Big(r\log\big(d\big)+\log\big(\frac{1}{\epsilon}\big) \Big)}&\text{ when } \sqrt{d/2}\leq r \leq d/3\label{eq:4}
\end{align}
and $|\cup_{x\in S}B(x,cr)|<2^{d-1}$.
\begin{proof}


Recall definition \ref{def:EDSAM}. Given a set $S$ of size $n$, a valid filter could be constructed by storing at most $n$ balls, $A_1,..,A_n$, selected so that:
\begin{enumerate}  
\item   For each $x\in S$ there is some $A_i$ such that $x\in A_i$.
\item   And the distance from $x$ to the edge of $A_i$ is at least $r$. \alertF{is edge of a ball defined?}
\item   $|\cup A_1,..,A_n|\leq \big(2^d-\cup_{x\in S}B(x,cr)\big)\epsilon+\cup_{x\in S}B(x,cr)$ 
\end{enumerate}
  
A query $q$ would be answered positively if there is some $A_i$ such that $q\in A_i$ and otherwise negatively.
We see that the first two requirements guarantee there will no false negatives, and the third that there won't be too many false positives.

We want to choose the largest $A_i$ balls possible without breaking the third requirement.
Assuming all $A_i$ have the same volume it would be:
\[
  |A_i|=(2^d-\cup_{x\in S}B(x,cr))\frac{\epsilon}{n}+B(cr)\geq 2^{d-1}\frac{\epsilon}{n},    
\]
if we assume that the total space covered by $\cup_{x\in S}B(x,cr)$ is less than $2^{d-1}$.


We will represent each ball $A_i=B(q_a,r_a)$ by a smaller ball $A_i^{-r}=B(q_a,r_a-r)$, so that if $x\in A_i^{-r}$ it fulfills both requirements.

The rest of the proof will progress as follows: First we will determine how large $A_i^{-r}$ can be, and we will then bound the size of a covering of the space by such balls.
An upper bound on storage is then given by the size of representing a specific choice of $n$ balls from the covering.

To find the radius of $A_i$ we want to select an $\epsilon/n$ fraction of the $d'=d-1$ dimensional hamming cube in a ball.
We can use the basic fact about the relationship bewteen the hamming ball and the Binonimal distribuition:

  \begin{lemma}[Hamming ball volume]
    \label{lem:BallVolume}
    By the definition of the radius $r\geq 0$ ball in $d$ dimensional hamming space: \alertF{The proof shouldn't be inside a lemma/theorem statement, even if trivial.}

    \[|B(r)|=\sum_{i=0}^{r}{d \choose i}=2^d\Pr[X\leq r] \text{ for } X\sim B(d,1/2)\]
where $B(d,p)$ is the binomial distribution.
\end{lemma}
    
This is usefull since we have thight bounds for the binomial distribution.
Particularly:
\begin{lemma}[Chernoff Bound]
  \label{lem:Chernoff}
  Let $X\sim B(d,1/2)$:

  \[
    \Pr[X\leq \frac{d}{2}-a]\leq e^{-2a^2/d}\text{ for } 0\leq a \leq d/2
    \]
\end{lemma}

So it's safe to set the radius of $A$ to at least $d/2-a$ where $a=\sqrt{\frac{d'\log(n/\epsilon)}{2}}$ since:
\[
  |B\big(\frac{d'}{2} - a\big)|=2^{d'}\Pr\Bigg[X\leq \mu - \sqrt{\frac{d'\log(n/\epsilon)}{2}}\Bigg]\leq 2^{d'}\epsilon/n
\]
Where $\mu = \E[X] = \frac{d'}{2}$.
We can express the radius of $A$ in terms of the number, $\lambda_a=\sqrt{2\log(n/\epsilon)}$, of standard deviations $X$ is from $\mu$.
Recall that the standard deviation for $B(d',0.5)$ is $\sqrt{d'}/2$, so the radius of $A^{-r}$ is at least:

\[
  \mu-(\lambda_a)\frac{\sqrt{d'}}{2}-r
\]

If we represent $r$ as a number of standard deviations,$\lambda_r=2r/\sqrt{d'}$, we find that the radius of $A^{-r}$ is at least:

\[
  \mu-(\lambda_a+\lambda_r)\frac{\sqrt{d'}}{2}
\]

Here's Berry-Essen:
  \begin{lemma}[Berry-Esseen]
    \label{lem:BerryEsseen}
    Let $X\sim B(d,1/2)$ and $x\in \BO{1}$:
\[
    \Phi(-x)-\frac{C}{\sqrt{d}}\leq\Pr[X\leq \frac{d}{2}-x\frac{\sqrt{d}}{2}]\leq \Phi(-x)+\frac{C}{\sqrt{d}}
  \]

  Where $\Phi(x)$ is the CDF of $\mathcal{N}(d/2,\sqrt{d}/2)$.
  $0.409732..\leq C \leq 0.4215$ by \cite{Nagaev2011}.
\end{lemma}
 
Now by lemma \ref{lem:BerryEsseen}:


\alertF{You should be sure that $C/\sqrt{d}$ is really negligible and not larger than $\Phi(x)$ for very small values of $x$ (I had this problem in my proof). Note that I use Berry-Esseen in the signature: if this section remains in the paper, we should not introduce Berry-Essen twice. 
Also I think it is not needed to use in a conference paper  full lemmas to introduce Chernoff bounds and Berry Esseen since they are well known (at least Chernoff bounds!).
}

\alertF{There is a big discontinuity here since the proof moved from a combinatorial approach to a probabilistic one. You should add more explanations.}

\begin{align}
  \Pr[X\leq\mu-(\lambda_a+\lambda_r)\sqrt{'d}/2]\approx  \frac{1}{\sqrt{2\pi}}\int_{-\infty}^{-\lambda_a-\lambda_r}e^{-t^2/2}dt=\\
    \frac{1}{\sqrt{2\pi}}\int_{-\infty}^{-\lambda_a}e^{-t^2/2}dt-\frac{1}{\sqrt{2\pi}}\int_{\lambda_a-\lambda_r}^{\lambda_a}e^{-t^2/2}dt)
\end{align}

Again by \ref{lem:BerryEsseen} and \ref{lem:Chernoff}:
\[
  \frac{1}{\sqrt{2\pi}}\int_{-\infty}^{-\lambda_a}e^{-t^2/2}dt\approx\Pr[X\leq \mu-\lambda_a\frac{d'}{2}]\leq\epsilon/n
\]

So by inserting:
\[
  \Pr[X\leq\mu-(\lambda_a+\lambda_r)\sqrt{d'}/2]\approx \epsilon/n - \frac{1}{\sqrt{2\pi}}\int_{-\sqrt{2\log(n/\epsilon)}-\lambda_r}^{-\sqrt{2\log(n/\epsilon)}}e^{-t^2/2}dt
\]

Simplifying and inserting $\lambda_r=2r/\sqrt{d'}$ we get:

\[
 \frac{|A_i^{-r}|}{2^{d'}}\approx \epsilon/n-1/2\Big(\text{Erf}(\frac{\sqrt{2}r}{\sqrt{d'}}+\sqrt{n/\epsilon})-\text{Erf}(\sqrt{n/\epsilon})\Big)
\]


Lets first look the the case where the volume is dominated by $\epsilon/n$, looking at the error function this happens if $\sqrt{n/\epsilon}$ is larger than $\approx 2$\jnote{This seems like a too relaxed bound. eps should be smaller than that i think}, no matter how large $r$ is, or if $\sqrt{n/\epsilon}$ is around $1$ or smaller i.e. $\epsilon\approx 1/n$ if $r<<\sqrt{\frac{d'}{2}}$.
So for $r<\sqrt{\frac{d-1}{2}}$ we will use $|A_i^{-r}|\in\BOM{2^{d-1}\epsilon /n}$

If the loss of volume from $r$ is substantial we can give another bound on the volume of $A_i^{-r}$:
\begin{lemma}
\label{lem:sphere in spheres}
Given a hamming ball $A=B_d(C_a,r_a)$ and a point $x\in A$. Let $d\geq r$.
\begin{equation}
\forall r<r_a\exists \lambda \text{ such that } B_d(\lambda,r)\subseteq A \text{ and } x\in B_d(\lambda,r)
\end{equation}
\begin{proof}
Take $XOR(x,C_a)$ and for the $r$ first non-zero entries flip the corresponding entry in $x$. Call the resulting vector $\lambda$. If $|XOR(x,C_a)|<r$ let $\lambda = C_a$.
Now $D(x,\lambda )\leq r$ so $x\in B(\lambda ,r)$. 
At the same time $D(C_a,\lambda )\leq r_a-r$ so the distance between $C_a$ and any point on $B(\lambda, r)$ is at most $r_a$.
Therefor $B(\lambda,r)\subseteq A$.
\end{proof}  
\end{lemma}

\begin{lemma}
\label{lem:sphere_contains}
A $d$ dimensional hamming sphere $A$ of radius $r_a$ can fully contain at least 
\begin{equation}
\frac{|A|}{\sum_{i=0}^r{d \choose i}}
\end{equation}
spheres of radius $r\leq r_a$.

\begin{proof}
Let $\lambda$ denote the set of center points of radius $r$ spheres fully contained in $A$. 
Since every point in $A$ lies within radius $r$ of some point in $\lambda$ (by lem.~\ref{lem:sphere in spheres}) we have $|\lambda|\sum_{i=0}^{r}{d \choose i}\geq |A|$.
\end{proof}
\end{lemma}

So for $r\geq \sqrt{\frac{d-1}{2}}$ we can use $|A_i^{-r}|$ is $\BOM{\frac{2^{d'}}{\sum_{j=0}^r{d \choose j}}}$.

To upper bound the size of the datastructure we will first determine how large a covering of the entire hamming space $\{0,1\}^d$ will be in these two settings of $A_i^{-r}$.

\begin{lemma}
\label{lem:random_covering}
There exists a covering of the $\{0,1\}^d$ space using $d2^d/V$ sets of volume $V$.
\begin{proof}
If we place $t$ sets at random the probability that a random point from $\{0,1\}^d$ is not covered is 
\begin{equation*}
(1-\frac{V}{2^d})^t\leq e^{-\frac{V}{2^d}t}
\end{equation*}
So by the union bound the probability that any point is left uncovered is bounded by
\begin{equation*}
2^de^{-\frac{V}{2^d}t}\leq 0.8
\end{equation*}
If we set $t=d\frac{2^d}{V}$.
\end{proof}
\end{lemma}

If we want a valid datastructure for all possible inputs, by lemma \ref{lem:random_covering} theres is some covering, $C$, of the space possible where the number of such balls is:
\begin{align}
   |C|&=d\frac{2^d}{|A_i^{-r}|}\rightarrow\\
      |C|&\leq\frac{dn}{\epsilon}\text{ for } r<\sqrt{(d-1)/2}\\
  |C|&\leq\frac{d2(ed/r)^rn}{\epsilon}\text{ for } \sqrt{(d-1)/2}<r<d/3 
\end{align}

 When processing an input set $S$ of size $n$ we would need to find and store the indexes associated with at most $n$ balls containing a full $B(x,r)$ associated with each $x\in S$. 
So a valid data structure is simply to distinguish which size $n$ subset corresponds to $S$ , requiring space:

\[
  \BO{\log{{|C|\choose n}}}=
\begin{cases}
  \BO{n\Big(\log\big(d\big)+\log\big(1/(\epsilon\big) \Big)}\text{ for } r<\sqrt{(d-1)/2}\\
  \BO{n\Big((r+1)\log\big(d\big)+\log\big(1/(\epsilon\big) \Big)}\text{ for } \sqrt{(d-1)/2}<r<d/3
\end{cases} 
\]

Note that we rely on a non-constructive existence proof for the cover, however for a given $d$ a more efficient cover will often be available.
\end{proof}
\end{theorem}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> dmq/definition.tex <==
 \section{Locality Sensitive Approximate Membership}
\subsection{Worst case error version (LSAM)}
For $r>0$, $\epsilon\in[0,1]$,$c\geq 1$. 
Given a set $S\subseteq X$,  a datastructure solves the $(c,r,\epsilon)$-LSAM problem if when queried with some $q\in X$ it reports: 

\begin{itemize}
\item \emph{Yes} if $D(q,S)\leq r$. 
\item  \emph{No} with probability at least $1-\epsilon$  if $D(q,S)\geq cr$.
\end{itemize}

If $r<D(q,S)<cr$ the datatstructure may give any answer.

The problem is well defined for any metric space $(X,D)$. We will focus on addressing it in $(\{0,1\}^d,\mathbb{H})$.

\subsection{Expected error version (ELSAM)}

Since the purpose of the datastructure is to discriminate points based on their proximity to points in $S$ it seems natural to allow the error probability to depend on this. 
We allow the structure to fail more often on near than far points and only promise bounds on the expected error:\\
For  $r>0$, $\epsilon \in [0,1]$. 
Given a set $S\subseteq X$ a datastructure solves the $(r,\epsilon)$-ELSAM  problem if  when queried with some $q\in X$ it reports: 

\begin{itemize}
\item \emph{Yes} if $D(q,S)\leq r$. 
\item  \emph{No} with expected probability at least $1-\epsilon$  if $D(q,S)> r$.
\end{itemize}

Where the expectation is over $q\in X\setminus\{\cup_{x\in S} B(x,r)\} $. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> dmq/makefile <==
SHELL = bash
SRC = $(wildcard illustrations/*.mp)
SUBSRC = $(patsubst illustrations/%.mp,%.mp,$(SRC))

mp :
	cd illustrations;for file in $(SUBSRC) ; do \
		mpost -tex=latex $$file ; \
	done

pdf : mp $(SRC)
	pdflatex main.tex
	pdflatex main.tex
	okular main.pdf

clean :
	$(RM) main.pdf *.log *.aux *.out *.bbl *.blg *.toc *.nav main.snm
	mv illustrations/*.mp .
	$(RM) illustrations/*
	mv *.mp illustrations/



==> dmq/notation.tex <==
\subsection{Notation}
\begin{itemize}
\item In a $(X,D)$ metric space, given a set $S\subseteq X$ and a point $q\in X$ let $D(q,S)$ = $\min_{x\in S}D(q,x)$.
\item Let $B_d(r)$ denote a radius $r$ hamming ball in $d$ dimensions, and $B_d(x,r)$ be a radius $r$ ball centered in $x$.
\item Let $S_d(r)$ denote the surface area of $B_d(r)$.
\item $\mathbb{H}$ is the Hamming distance.
\end{itemize}


==> dmq/overview.tex <==
\subsection{Average case}

In the average case we guarantee that at most an $\epsilon$ fraction of the points $\notin \{\cup_{x\in S}B(x,r)\}$ are accepted. 
$$
\BO{n\Big(r\log\big(d\big)-\log\big(\frac{\epsilon}{n}+\frac{(1-\epsilon){d \choose r}}{2^{d}}\big) \Big)}$$
 when $r\leq d/2-\sqrt{d}$.

$$\Omega \Big( n\big(r \log(d) - \log (\epsilon+ \frac{n {d \choose r}}{2^{d-1}}) \big)\Big)$$
where $r<d/3$.

\subsection{Worst case}

In the worst case we guarantee that any point $\notin \{\cup_{x\in S}B(x,cr)\}$ is accepted w.p $\leq \epsilon$.

\subsubsection{Lower bound}
Based on the promised existence of error correctiong codes with the properties:

\begin{itemize}
\item $1/(r\epsilon)^2$ code words
\item Each of length $d/k$
\item And weight $r/k$
\item Minimum distance betwenn codewords $r(c-1)$
\end{itemize}

Two codewords compared by table 1:
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> dmq/prior.tex <==
\subsection{Prior work}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

There is some prior work in membership structures that incorporate locality \cite{Kirsch}, \cite{Hua2012}.
Efforts here have been focused on constructing Bloom filters\cite{Qiao2014},\cite{Carter1978} but using locality sensitive hash functions\cite{Gionis99} to make the filters distance sensitive. 

However one of the main benefits of Bloom filters is the lack of false negatives. 
Having only false positives makes Bloom filters useful in many practical scenarios where a few false positives are acceptable, but avoiding false negatives crucial.
Unfortunately the hash functions used in both \cite{Kirsch} and \cite{Hua2012} introduce false negatives.


==> dmq/tmp.tex <==
\renewcommand{\d}{\kappa}
In this section we propose a data structure for  answering $(c,r,\epsilon)$-LSAM queries  on $n$ input vectors.
We initially introduce the notion of signature, that is a function mapping a $d$-dimensional binary vector into $\BO{???}$ bits. 
Then, we show that storing the signature of the $n$ input vertexes gives a data structure for LSAM queries requiring $\BO{}$ query time and $\BO{}$ total space. 
We will later show how to reduce the query time to $\BO{???}$ by increasing the space complexity by a $\BO{???}$.

Let\footnote{We denote with $[n]$ the set $\{0,1\ldots,n-1\}$, with $X^n$ the $n$-fold cartesian product of set $X$, and with $2^X$ the power set of set $X$.}
 $R:[d]\rightarrow [\d]^\Delta$ be a function assigning uniformly and independently at random $\Delta$ values in $[\d]$ to every $x\in[d]$, where  
$$\Delta=\left \lceil \frac{4\log (4/\epsilon)}{(c-1)r}\right \rceil \quad \textnormal{and}\quad
\d=(c+1) \Delta r = \BO{\frac{\log (1/\epsilon)}{(c-1)}+cr
}.$$
Let $L:[\d]\rightarrow 2^{[d]}$ be the inverse of $R(\cdot)$, that is the function returning for each $y\in[\d]$ the values $x\in[d]$ such that $y\in R(x)$. 
Finally, we set $\ell:[\d]\rightarrow [d]$ to denote the sizes of the sets returned by $L$, that is $\ell(y)=|L(y)|$.
Intuitively, function $R(\cdot)$ denotes a bipartite expander graph connecting $d$ left nodes with degree $\Delta$ to the $\d'$ right nodes.

From   functions $R(\cdot)$ and $L(\cdot)$, we construct the signature of a given $d$-dimensional boolean vector $p$ as follows.
We define $f_i:\{0,1\}^{\d}\rightarrow \{0,1\}^d$, with $i\in[\d]$, as $f_i(p)=(p_{l_{i,0}}, \ldots, p_{i,l_\ell(i)-1})$, where $L(i)=(l_{i,0},\ldots,l_{i,\ell(i)-1})$, and we let $F(p)=(f_0(p),\ldots, f_{\d-1})$. 
Finally, we denote with  $h_i:\{0,1\}^{\d}\rightarrow \{0,1\}^\rho$, with $i\in [\d]$ and $\rho=\log(2(c+1)/(c-1))$, a 2-independent hash function.
We assume that the random functions $R(\cdot), h_0(\cdot), \ldots, h_{\kappa-1}$ are independent.
The \emph{$(c,r,\epsilon)$-signature} of a vector $p$ is then the vector $H(p)=(H_i(p),\ldots H_{\d-1}(p))=(h_0(f_0(p)),\ldots h_{\d-1}(f_{\d-1}(p))$.

Consider two points $p$ and $q$ and their signatures $H(p)$ and $H(q)$. 
When $d(q,p)\leq r$, signature $H(p)$ and $H(q)$ cannot differ on more than $\Delta r$ positions:  
indeed, each bit position where $p$ and $q$ differ affects at most $\Delta$ functions $f_i(\cdot)$, and then there cannot be more than $\Delta r$ differences between $H(p)$ and $H(q)$.
When $d(p,q)\geq cr$, we claim that $H(p)$ and $H(q)$ differ on at least $\Delta r$ positions with probability larger than $1-\epsilon$. For simplicity, denote with $x_0, \ldots, x_{cr-1}$ the bit positions where $p$ and $q$ differ.
This property fails in two cases: 
\begin{enumerate}
\item \textit{Expansion failure:} 
Bit positions $x_0, \ldots, x_{cr-1}$ affect less than $\Delta r$ functions $f_i()$: 
this implies that there cannot be more than $\alpha \Delta r$ differences between $F(q)$ and $F(p)$, and hence between $H(q)$ and $H(p)$.
For the sake of the analysis, we use a more broad definition of expansion failure, which includes the case where $x_0, \ldots, x_{cr-1}$ affect less than $\alpha \Delta r$ functions $f_i()$, with $\alpha=(c+1)/2$. 

\item \textit{Collision failure:} Assume there is no  expansion failure: then, there are at least $\alpha \Delta r$ different positions between $F(p)$ and $F(q)$. 
If at least $(\alpha-1)\Delta r$ hash functions associated with  these positions collide for $p$ and $q$ (i.e., $h_i(f_i(q))=h_i(f_i(p))$ when $f_i(q)\neq f_i(p)$), then the number of different positions between $H(q)$ and $H(p)$ is less than $\Delta r$.
\end{enumerate}

The next two lemmas show that the expansion and collision failures  happen with probability $\epsilon/2$ each. This implies that, when $d(p,q)\geq cr$, the signature $H(p)$ and $H(q)$ differ on at least $\Delta r$ positions with probability at least $1-\epsilon$.
\begin{lemma}
The expansion failure happens with probability at most $\epsilon/2$.
\end{lemma}
\begin{proof} 
It is convenient to consider  the bipartite expander graph underlying function $R(\cdot)$: it is easy to see that the expansion failure is equivalent to the case where the $c\Delta r$ edges from the given $cr$ left nodes $x_0,\ldots x_{cr-1}$ touch less than $\alpha \Delta r $ right nodes, where $\alpha=(c+1)/2$. Denote with $e_0,\ldots e_{c\Delta r-1}$ the edges of $x_0,\ldots x_{cr-1}$, and assume without loss of generality that edge $e_{i+1}$ is (independently) randomly assigned to the right nodes after node $e_{i}$ for each $i\in [c\Delta r]$. We say that edge $e_i=(x,y)$ is a \emph{starting edge} if $i=0$ or if the right node $y$ is not adjacent to edges $e_0,\ldots, e_{i-1}$, or if $i=0$. Note that there is at most one starting edge for each right node. 

Let $E_j$ be the event where exactly $j$ right nodes are touched by the $c\Delta r$ edges, and let $E'_{i_0,\ldots, i_{j}}$ be the event where edges $e_{i_0},\ldots, e_{i_{j}}$ are starting nodes.
\begin{align*}
\Pr[E_j] &= \sum_{\forall i_0,\ldots i_{j}} \Pr[E_j | E'_{i_0,\ldots, i_{j}} ] \Pr[ E'_{i_0,\ldots, i_{j}} ] \\
& \leq \sum_{\forall i_0,\ldots i_{j}} \left(1 \frac{m-1}{m}\ldots \frac{m-i}{m} \right)
 \left(\frac{i}{\d}\right)^{c\Delta r-i} \Pr[ E'_{i_0,\ldots, i_{j}} ]
\leq \left(\frac{i}{\d}\right)^{c\Delta r-i}
\end{align*}
where the first parenthesis gives the probability that the $i$ starting edges are assigned to different right nodes, and the second one the probability that the remaining $c\Delta r-i$ edges do not affect other right nodes.
By summing above the $\alpha \Delta r$ possible values of $j$, we get 
\begin{align*}
\Pr[\textnormal{Expansion failure}]&=\sum_{i=1}^{\alpha \Delta r} \Pr[E_i] \leq 
\sum_{i=1}^{\alpha \Delta r}  
\left(\frac{i}{\d}\right)^{c\Delta r-i}
\leq
\sum_{i=1}^{\alpha \Delta r}  
\frac{1}{2î}\left(\frac{\alpha \Delta}{\d}\right)^{(c-\alpha)\Delta r} 
\\
&\leq  2 \left(\frac{1}{2}\right)^{(c-\alpha)\Delta r}
= 2 
\left(\frac{1}{2}\right)^{(c-1)\Delta r/2}
\leq \epsilon/2.
\end{align*}
where the last step follows since $\d\geq (c+1) \Delta r$ and $(c-1)\Delta r\geq 2 \log (4/\epsilon)$.
\end{proof}

\begin{lemma}
If there is no expansion failure, then the collision failure happens with probability at most $\epsilon/2$.
\end{lemma}
\begin{proof}
Since there is no expansion failure, we assume that $F(q)$ and $F(p)$ differ on at least $\alpha \Delta r$ positions, say $f_0(\cdot),\ldots f_{\alpha \Delta r-1}(\cdot)$, with $\alpha=(c+1)/2$.
Let denote with $W_i$, with $i\in [ \alpha \Delta r]$, the random variable with value $1$ if $h_i(f_i(q))=h_i(f_i(p))$ and $0$ otherwise.
A collision failure requires that $W=\sum_{i=0}^{\alpha \Delta r-1} W_i \geq (\alpha-1)\Delta r$ in order to reduce the number of different positions between $H(p)$ and $H(q)$ below $\Delta r$.

We claim that $\Pr[W \geq (\alpha-1)\Delta r]\leq \epsilon/2$.
Random variables $W_i$ are independent and each hash function $h_i(\cdot)$ has collision probability $1/2^\rho=(c-1)/(2(c+1))$. 
Let the expected value of $W$ be $\mu =  \alpha \Delta r/\rho$ and let $\beta=(\alpha-1)\Delta r/\mu -1$. 
With a Chernoff bound, we get
\begin{align*}
\Pr[\textnormal{Collision failure}]\leq 
\Pr[W \geq (\alpha-1)\Delta r] = \Pr[W \geq (1+\beta)\mu]  
\leq e^{-\beta\mu/2} \leq \epsilon/2.
\end{align*}
The last step follows since $1/2^\rho= (c-1)/(2(c+1))$ and $(c-1)\Delta  r\geq 4\log(2/\epsilon)$.
\end{proof}

A simple data structure for $(\epsilon, r, c)$-LSAM on $n$ points follow by storing the $(\epsilon/n, r,c)$ signature of the $n$ vectors.
Then, for each query $q$ the answer is returned by comparing $H(q)$ with every signature in the data structure. We get the following theorem.

\begin{theorem}
The above data structure requires 
$$S(n,r,c,\epsilon)= \BO{n\log \left(\frac{c}{c-1}\right)\left(\frac{c}{(c-1)}\log \left(\frac{n}{\epsilon}\right) +cr\right)}$$
total bits, and it  answers an $(\epsilon, r, c)$-LSAM  query $q$ on $n$ boolean vectors in  $S(n,r,c,\epsilon)/\log n$ time by using memory words of at least $\log n$ bits.
\end{theorem}
\begin{proof}
By an union bound, we have that the $n$ signatures do not fail with probability at least $1-\epsilon$ when compared with $q$.
Since each signature requires $\kappa=\frac{c}{(c-1)}\log \left(\frac{n}{\epsilon}\right) +cr$ sequences of $\rho=2(c+1)/(c-1)$ bits, the total data structure size follows.
The time bound follows by exploiting the fact that in an unit time it is possible to compare at least $\log n$ bits.
\end{proof}

It is interesting to analyze the space complexity under some special cases:
\begin{itemize}
\item If $1\leq c\leq 2$, $r=\BO{\log (1\epsilon)/(c-1)}$ and $\epsilon=1/n^{\BT{1}}$: the data structure uses $\BO{\frac{n}{c-1} \log (1/c-1) \log{1/\epsilon}}$ bits which is a factor $\log(1/c-1)$ from the optimal space bound.
\item 
If $c\geq 2$ and $\epsilon=1/n^{\BT{1}}$: the data structure uses $\BO{n\left(\log{1/\epsilon}+r\right)}$ bits, which matches a Bloom filter if $r$ is not too large.
\item TODO: comments on the dimension $d$, comparison with previous works.
\end{itemize}

TODO:
We now show that by setting $m=..$,... it is possible to obtain a data structure for LSMQ by concatenating the $n$ signatures of the $n$ input vector. For each query $q$, the answer is performed by comparing the $n$ signature with $H(q)$ as shown above. 
We get the following result.
\begin{theorem}
Given $n$ points $p$ and a query $q$, there exists a data structure that answer a LSAM query $q$ with false positive rate $\epsilon$ and approximation $c\geq 1$.
\end{theorem}
\begin{proof}

\end{proof}

==> fn/figures/beta-final.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1518){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(946,2332){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(946,3147){\makebox(0,0)[r]{\strut{} 1.3}}%
      \put(946,3961){\makebox(0,0)[r]{\strut{} 1.4}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1078,484){\makebox(0,0){\strut{} 0}}%
      \put(1841,484){\makebox(0,0){\strut{} 2}}%
      \put(2605,484){\makebox(0,0){\strut{} 4}}%
      \put(3368,484){\makebox(0,0){\strut{} 6}}%
      \put(4131,484){\makebox(0,0){\strut{} 8}}%
      \put(4895,484){\makebox(0,0){\strut{} 10}}%
      \put(5658,484){\makebox(0,0){\strut{} 12}}%
      \put(6421,484){\makebox(0,0){\strut{} 14}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}approximation achieved ($c$)}}}%
      \put(3940,154){\makebox(0,0){\strut{}points examined ($m$), with $\ell m=48$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}range/quartiles/median}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}sample mean}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}query-independent}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{beta-final.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> fn/figures/colors-final.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1518){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(946,2332){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(946,3147){\makebox(0,0)[r]{\strut{} 1.3}}%
      \put(946,3961){\makebox(0,0)[r]{\strut{} 1.4}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1078,484){\makebox(0,0){\strut{} 0}}%
      \put(2032,484){\makebox(0,0){\strut{} 5}}%
      \put(2986,484){\makebox(0,0){\strut{} 10}}%
      \put(3941,484){\makebox(0,0){\strut{} 15}}%
      \put(4895,484){\makebox(0,0){\strut{} 20}}%
      \put(5849,484){\makebox(0,0){\strut{} 25}}%
      \put(6803,484){\makebox(0,0){\strut{} 30}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}approximation achieved ($c$)}}}%
      \put(3940,154){\makebox(0,0){\strut{}projections and points examined ($\ell=m$)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}range/quartiles/median}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}sample mean}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}query-independent}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{colors-final.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> fn/figures/movies-final.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(814,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(814,1518){\makebox(0,0)[r]{\strut{}$1.1$}}%
      \put(814,2332){\makebox(0,0)[r]{\strut{}$1.2$}}%
      \put(814,3147){\makebox(0,0)[r]{\strut{}$1.3$}}%
      \put(814,3961){\makebox(0,0)[r]{\strut{}$1.4$}}%
      \put(814,4775){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \put(946,484){\makebox(0,0){\strut{}$0$}}%
      \put(1922,484){\makebox(0,0){\strut{}$5$}}%
      \put(2898,484){\makebox(0,0){\strut{}$10$}}%
      \put(3875,484){\makebox(0,0){\strut{}$15$}}%
      \put(4851,484){\makebox(0,0){\strut{}$20$}}%
      \put(5827,484){\makebox(0,0){\strut{}$25$}}%
      \put(6803,484){\makebox(0,0){\strut{}$30$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}approximation achieved ($c$)}}}%
      \put(3874,154){\makebox(0,0){\strut{}projections and points examined ($\ell=m$)}}%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}range/quartiles/median}}%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}sample mean}}%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}query-independent}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{movies-final.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> fn/figures/nasa-final.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1518){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(946,2332){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(946,3147){\makebox(0,0)[r]{\strut{} 1.3}}%
      \put(946,3961){\makebox(0,0)[r]{\strut{} 1.4}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1078,484){\makebox(0,0){\strut{} 0}}%
      \put(2032,484){\makebox(0,0){\strut{} 5}}%
      \put(2986,484){\makebox(0,0){\strut{} 10}}%
      \put(3941,484){\makebox(0,0){\strut{} 15}}%
      \put(4895,484){\makebox(0,0){\strut{} 20}}%
      \put(5849,484){\makebox(0,0){\strut{} 25}}%
      \put(6803,484){\makebox(0,0){\strut{} 30}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}approximation achieved ($c$)}}}%
      \put(3940,154){\makebox(0,0){\strut{}projections and points examined ($\ell=m$)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}range/quartiles/median}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}sample mean}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}query-independent}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{nasa-final.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> fn/figures/normal-final.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1518){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(946,2332){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(946,3147){\makebox(0,0)[r]{\strut{} 1.3}}%
      \put(946,3961){\makebox(0,0)[r]{\strut{} 1.4}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1078,484){\makebox(0,0){\strut{} 0}}%
      \put(2032,484){\makebox(0,0){\strut{} 5}}%
      \put(2986,484){\makebox(0,0){\strut{} 10}}%
      \put(3941,484){\makebox(0,0){\strut{} 15}}%
      \put(4895,484){\makebox(0,0){\strut{} 20}}%
      \put(5849,484){\makebox(0,0){\strut{} 25}}%
      \put(6803,484){\makebox(0,0){\strut{} 30}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}approximation achieved ($c$)}}}%
      \put(3940,154){\makebox(0,0){\strut{}projections and points examined ($\ell=m$)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}range/quartiles/median}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}sample mean}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}query-independent}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{normal-final.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> fn/figures/uniform-final.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,1518){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(946,2332){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(946,3147){\makebox(0,0)[r]{\strut{} 1.3}}%
      \put(946,3961){\makebox(0,0)[r]{\strut{} 1.4}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1078,484){\makebox(0,0){\strut{} 0}}%
      \put(2032,484){\makebox(0,0){\strut{} 5}}%
      \put(2986,484){\makebox(0,0){\strut{} 10}}%
      \put(3941,484){\makebox(0,0){\strut{} 15}}%
      \put(4895,484){\makebox(0,0){\strut{} 20}}%
      \put(5849,484){\makebox(0,0){\strut{} 25}}%
      \put(6803,484){\makebox(0,0){\strut{} 30}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}approximation achieved ($c$)}}}%
      \put(3940,154){\makebox(0,0){\strut{}projections and points examined ($\ell=m$)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}range/quartiles/median}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}sample mean}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}query-independent}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{uniform-final.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> fn/makefile <==
SHELL = bash
SRC = $(wildcard *.mp)

mp :
	for file in $(SRC) ; do \
		mpost -tex=latex $$file ; \
	done

pdf : mp $(SRC)
	pdflatex main.tex
	bibtex main
	pdflatex main.tex
	pdflatex main.tex
	pdflatex main.tex
	okular main.pdf

clean :
	$(RM) main.pdf *.log *.aux *.out *.bbl *.blg *.toc *.nav main.snm *.1 *.2 *.3


==> makefile <==
SHELL = bash
SRC=$(wildcard mpsrc/*.mp)
SUBSRC=$(patsubst mpsrc/%.mp,%.mp,$(SRC))
NAMES=$(patsubst mpsrc/%.mp,%,$(SRC))
define PNGTEXT
outputformat := "png";
hppp:=0.1;
vpp:=0.1;
outputtemplate := "%j.%o";
warningcheck :=0;
endef
export PNGTEXT

print-%  : ; @echo $* = $($*)

mp:
	cd mpsrc;./compile.sh;

png:
	mkdir png	
	cd src;for file in $(SUBSRC) ;do \
		sed '1 i warningcheck:=0;' $$file > png_$$file;\
		sed -i '1 i outputtemplate := "%j_%c.%o";' png_$$file;\
		sed -i '1 i vppp:=0.2;' png_$$file;\
		sed -i '1 i hppp:=0.2;' png_$$file;\
		sed -i '1 i outputformat := "png" ;' png_$$file;\
		mpost -tex=latex png_$$file;\
		$(RM) png_$$file*;\
		$(RM) *.log ;\
		rename 's/png_//' *.png ;\
		mv *.png ../png ;\
	done
	mv src/* .
	mv *.mp src

html: png
	mkdir html;
	echo "<html><title>My metapost figues</title><body>" > html/metapost.html
	for file in png/*png ; do \
	echo "<img src=\"../"$$file"\">" >> html/metapost.html;\
	done
	echo "</body></html>" >> html/metapost.html	


pdf : mp
	pdflatex thesis.tex
	pdflatex thesis.tex

update : mp $(SRC)
		./tex/texgen $(SRC)
		pdflatex ./tex/main.tex


clean :
	cd figures;$(foreach file,$(NAMES),$(RM) $(file).*)


==> simfilter/_region_.tex <==
\message{ !name(simfilter.tex)}
\message{ !name(algorithm.tex) !offset(168) }
The bound on the depth of the Chosen Path Tree for $x$ explored by the \cpsj algorithm in Lemma
\message{ !name(simfilter.tex) !offset(-4) }


==> simfilter/experiments_old.tex <==
%!TEX root = simfilter.tex
%-------------------------------------------
\section{Experiments}
%-------------------------------------------
We run on the implementations of Chosen Path Similarity Join (CP), MinHash LSH (MH), BayesLSH (BLSH), and AllPairs (ALL) for similarity thresholds $\lambda \in \{0.5, 0.6, 0.7, 0.8, 0.9 \}$.

All experiments were run on an Intel i7-4790 CPU at 3.60GHz with $8192$kB L$3$, $256$kB L$2$ and $32$kB L$1$ cache and $32$GB of RAM.
Since a single experiment is always confined to a single CPU core we ran several experiments in parallel~\cite{Tange2011a} to better utilize the time.

\textbf{Recall.}
In our experiments we aim for a recall of at least $90\%$ for the approximate methods. 
In order to achieve this for the Chosen Path Similarity Join and MinHash LSH algorithms we perform a number of repetitions after the preprocessing step, stopping when the desired recall has been achieved.
Note that the preprocessing step only has to be performed once for each data set, and can be re-used


\subsection{Data sets.}
The performance is measured across $10$ real world data sets along with $2$ synthetic data sets, 
provided by the authors of~\cite{Mann2016} where descriptions and sources for each data set can also be found\footnote{We have renamed the SPOT datset to SPOTIFY}.
For completeness some central characteristics of the datasets from~\cite{Mann2016} are given in table~\ref{tab:datasets}.
\begin{table}
  \begin{tabular}{lrrr}
    Dataset & \# sets/$10^6$ & avg. set size & \# tokens/$10^3$\\\toprule
    AOL & $10 $ & 3.0 & $3900$\\
    BMS-POS & $0.32 $ & $9.3$& $1.6$\\
    DBLP & $0.1$ & $82.7$ & $6.8$\\
    ENRON & $0.25$ & $135.2 $& $1100$\\
    FLICKR & $1.2 $ &$10.1$ & $81$\\
    LIVEJ & $3.1$ &$36.4$& $7500$\\
    KOSARAK & $0.61 $ &$11.9$& $41$\\
    NETFLIX & $0.48 $ &$209.5$&$18$\\
    ORKUT & $2.7 $ &$119.7$&$8700$\\
    SPOTIFY & $0.44 $ &$12.8$&$760$\\
    UNIFORM & $0.1$ &$10.0$&$0.2$\\
    ZIPF & $0.1 $& $50.0$&$102$
  \end{tabular}
  \caption{Datasets~\protect\cite{Mann2016}}
    \label{tab:datasets}
\end{table}
Experiments are run on versions of the datasets where duplicate records are removed and any records containing only a single token are ignored.
The data sets display a varity of internal structure which has strong impact on the performance of the different algorithms.
For each data set a self join is performed and the resulting pairs are verified and stored.

\subsection{Choosing parameters}


\subsection{Performance measures}

\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{speed.pdf}
  \caption{Relative Speed compared to ALL}
  \label{fig:speed}
\end{figure}


\subsubsection{Runtime}

We measure \emph{join time}, the time spent by the algorithms for performing a similarity self-join for each data set.
This excludes all parsing and tokenizing and any sorting, drawing of psudo-random numbers or skectching of records performed by the algorithms.
To make comparisons more accurate we also instruct prefix-based algorithms to build indexes as part of the preprocessing phase rather than incrementally throughout the joining phase.
\emph{Join time} measures the time spent between having a ready preprocessed dataset read into memory and outputting a list of results.
For the prefix length based algorithms tested this includes generating candidates, filtering and verifying them.
For the \cpsj algorithm this includes recursivly splitting the data into buckets, processing the buckets into pairs and verifying them.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.4\textwidth]{Time_NETFLIX.pdf}
  \caption{NETFLIX self-join time comparison.}
    \label{fig:netflix}
\end{figure}

\begin{figure}[h]  \centering
  \includegraphics[width=0.4\textwidth]{Time_ORKUT.pdf}
  \caption{ORKUT self-join time comparison.}
  \label{fig:orkut}
\end{figure}
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.4\textwidth]{dedupitems.png}
%   \caption{Enron}
%\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=0.4\textwidth]{Time_FLICKR.pdf}
  \caption{FLICKER self-join time comparison.}
  \label{fig:flickr}
\end{figure}
% \begin{figure}
%   \centering
%   \includegraphics[width=0.4\textwidth]{rm-s100000.png}
%   \caption{Uniform 0.05}
% \end{figure}



\begin{table*}[t]
  \centering
\csvreader[tabular=lrrrrrrrrrr
, table head=&\multicolumn{2}{c}{Threshold $0.5$}&\multicolumn{2}{c}{Threshold $0.6$}&\multicolumn{2}{c}{Threshold $0.7$}&\multicolumn{2}{c}{Threshold $0.8$}&\multicolumn{2}{c}{Threshold $0.9$}\\\toprule Dataset & Time &Recall & Time & Recall& Time & Recall &  Time &Recall& Time & Recall \\\hline\hline
, table foot=\hline, head to column names
, late after line=\\
, late after last line =\\\bottomrule]{table2.csv}{}
{\Dataset& \JoinA & \ResultsA& \JoinB & \ResultsB& \JoinC &\ResultsC& \JoinD &\ResultsD& \JoinE &\ResultsE}
\caption{All numbers show $\%$ versus ALL}
  \label{tab:comparison}
\end{table*}

The \emph{join time} measured for ALL on the datasets are in line with the results from~\cite{Mann2016}.
We observe slightly faster times, reflecting the higher CPU clock used for these experiments.

An overview of the comparison results is provided in Figure~\ref{fig:speed}. Most datasets experience significant speedups, most notably at lower thresholds.
Figure~\ref{fig:scatter} shows the relationship between \cpsj and ALL \emph{join time} for a representative selection of the datasets, we observe that higher speedups occur when ALL is slow.
\begin{figure}
  \includegraphics[width=0.4\textwidth]{scatter.pdf}
  \caption{Speed comparison}
  
  \label{fig:scatter}
\end{figure}
The datasets can be grouped into three categories in terms of the behavior of \cpsj vs ALL (see table~\ref{tab:comparison}).

For one group of datasets, NETFLIX (see Figure~\ref{fig:netflix}), ORKUT (see Figure~\ref{fig:orkut}), UNIFORM, DBLP, LIVEJ, ENRON and BMS-POS the \cpsj needs much less time than ALL, 
while retaining a recall much larger than the fraction of ALLs \emph{join time} spent.
The benefit is greatest for thresholds up to $0.7$, at higher thresholds ALL remains favorable for the tested datasets.
However the time spent for both algorithms at high threshold values is often significantly less than one second (see table~\ref{tab:ALL}) and it seems hard to bring much improvement for these datasets. It would be interesting future work to run the comparisons on datasets with larger set sizes where prefix filtering will still leave significant work, even at high thresholds.
Based one our experiments we expect the benefit of \cpsj to grow compared to ALL as set sizes grow, keeping other things equal.

The second group consists of KOSARAK and AOL. Here \cpsj is faster than ALL, but the recall drops at a similar rate or worse, 
leaving little benefit over ALL. We suspect that this is due to these sets containing very many similar points, we further elaborate on this in section~\ref{sec:candidates}.

The final group contains the FLICKR (see Figure~\ref{fig:flickr}) dataset, 
with SPOTIFY somewhere between group two and three. 
For this dataset \cpsj needs about twice the time while finding only around half the results. 
It seems both FLICKR and SPOTIFY are uniquely suited for prefix filtering because they contain very many rare tokens and have small average set sizes (see table DATASETS). 
This means that prefix filtering will only have to process very few, very short lists for each record.


\begin{table*}[t]
  \centering
    \label{tab:orkut}
\csvreader[separator=tab,tabular=crrrrrrr
, table head=&\multicolumn{2}{c}{All Pairs}&\multicolumn{4}{c}{Chosen Path}
\\\toprule Threshold & Candidates &Results & Precision\% & Pre-Candidates & Candidates & Results & Precision\% \\\hline\hline
, table foot=\hline, head to column names
, late after line=\\
, late after last line =\\\bottomrule]{kut.csv}{}
{\Threshold& \APCandidates & \APResults & \APResultsP & \CPPre& \CPCandidates &\CPResults& \CPResultsP}
\caption{ORKUT}
\end{table*}


\begin{table*}[t]
  \centering
\csvreader[separator=tab,tabular=crrrrrrr
, table head=&\multicolumn{2}{c}{All Pairs}&\multicolumn{4}{c}{Chosen Path}
\\\toprule Threshold & Candidates &Results & Precision\% & Pre-Candidates & Candidates & Results &Precision\% \\\hline\hline
, table foot=\hline, head to column names
, late after line=\\
, late after last line =\\\bottomrule]{kosarek.csv}{}
{\Threshold& \APCandidates & \APResults & \APResultsP & \CPPre& \CPCandidates &\CPResults& \CPResultsP}
\caption{KOSARAK}
  \label{tab:kosarak}
\end{table*}

\begin{table*}[t]
  \centering
\csvreader[separator=tab,tabular=crrrrrrr
, table head=&\multicolumn{2}{c}{All Pairs}&\multicolumn{4}{c}{Chosen Path}
\\\toprule Threshold & Candidates &Results & Precision\% & Pre-Candidates & Candidates & Results &Precision\% \\\hline\hline
, table foot=\hline, head to column names
, late after line=\\
, late after last line =\\\bottomrule]{netflix.csv}{}
{\Threshold& \APCandidates & \APResults & \APResultsP & \CPPre & \CPCandidates &\CPResults& \CPResultsP}
\caption{NETFLIX}
\label{tab:netflix}
\end{table*}


% \begin{table*}[t]
%   \centering
%   \label{tab:aol}
% \csvreader[separator=tab,tabular=crrrrrrr
% , table head=&\multicolumn{2}{c}{All Pairs}&\multicolumn{4}{c}{Chosen Path}
% \\\toprule Threshold & Candidates &Results & Precision\% & Pre-Candidates & Candidates & Results &Precision\% \\\hline\hline
% , table foot=\hline, head to column names
% , late after line=\\
% , late after last line =\\\bottomrule]{aol.csv}{}
% {\Threshold& \APCandidates & \APResults & \APResultsP & \CPPre& \CPCandidates &\CPResults& \CPResultsP}
% \caption{AOL}
% \end{table*}


\begin{table*}[t]
  \centering
\csvreader[separator=tab,tabular=crrrrrrr
, table head=&\multicolumn{2}{c}{All Pairs}&\multicolumn{4}{c}{Chosen Path}
\\\toprule Threshold & Candidates &Results &Precision\% & Pre-Candidates & Candidates & Results &Precision\% \\\hline\hline
, table foot=\hline, head to column names
, late after line=\\
, late after last line =\\\bottomrule]{flickr.csv}{}
{\Threshold& \APCandidates & \APResults & \APResultsP & \CPPre& \CPCandidates &\CPResults& \CPResultsP}
\caption{FLICKR}
    \label{tab:flickr}
\end{table*}

\subsubsection{Candidates}
\label{sec:candidates}
As a further performance measure we measure pre-candidate and candidate pairs.
For the prefix length based algorithms pre-candidates include all pairs generated from inverted indexes when using prefix and overlap size constraints, 
candidates are the subset of these points passing the various filters and deduplication employed. 
Since ALL employs no extra filters there is no difference between the two for ALL.
For the Chosen Path Similairty Join pre-candidates include all pairs generated in the recursive process using the overlap size constraints, 
the candidates are subset of pre-candidates remaining after filtering with sketches.
There are two ways to generate a pair in the Chosen Path Algorithm. 
A point can be selected in the sampling step and compared with all other points in the current bucket, or it can be generated when brute forcing all pairs in the leaf buckets.
When a pair is generated due to sampling, the pair is considered both a pre-candidate and a candidate. 
Since the point considered has already been selected based on having high sketch similarity, it is not again filtered by sketching.
If a pair is generated in a leaf bucket on the other hand, it might well be filtered out by distance sketching and be considered only a pre-candidate pair.

To be able to argue about the quality of randomized versus deterministic algorithms these performance measures are related to the number of verified results.

ORKUT and NETFLIX are examples of datasets where \cpsj achieves a large speedup over ALL.
This speed difference is clearly reflected in the number of candidates generated (see table~\ref{tab:orkut} and~\ref{tab:netflix}).
Even without sketching \cpsj generates much fewer candidate pairs than ALL, and crucially the number of results remains relatively large.
This means that \cpsj enjoys much higher precision than ALL pairs for most datasets, we consider this the main advantage of \cpsj.
Since \cpsj and ALL differ only in how candidates are generated, not how they are verified, it is clear that the difference in number of candidates represents an upper limit to the speedup achievable by \cpsj.
The cost of recursively splitting the points into buckets, deduplication and other bookkeeping in \cpsj is significant enough that the increased precision does not translate directly into speedup, there is still some room before reaching the limit defined by the precision increase.
Future work could focus on lowering these costs.
Our experiments indicate that a large fraction of the time spend during the \cpsj is spend in splitting buckets using a hashmap, it might be possible to improve this or other parts of the algorithm for a further speed gain.

Table~\ref{tab:kosarak} shows candidate generation results for KOSARAK, representing the middle group of sets where speed is improved, but recall drops at a similar or worse rate.
Looking at table~\ref{tab:kosarak} it seems a possible explanation is the very large amount of results returned for these sets.
It appears that the datasets contains many similar sets, the same holds for AOL. Even though \cpsj improves the precision the \cpsj candidate set is not much smaller than the ALL result set.
It is only possible for \cpsj to improve the \emph{join time} if precision is improved by shrinking the candidate set, not if it is improved by finding more results in similar sized sets.

For datasets where \cpsj has worse of similar performance to ALL, most notably FLICKR (see table~\ref{tab:flickr}), we notice that ALL already achieves an unusually high precision.
This indicated that the datasets are uniquely suited to prefix filtering, as noted in~\cite{Mann2016} this is likely due to the fact that they contain a large number of rare tokens.
The number of candidates generated by \cpsj for FLICKR is within a small factor, around $2$, of the number generated by ALL, 
while for datasets with the opposite structure, like NETFLIX, ALL generate several orders of magnitude more candidates than \cpsj.
This supports and explains the \emph{Join time} behaviour.

\subsubsection{Boosting recall}
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.4\textwidth]{Repeat_BMS-POS.pdf}
  \caption{Result set size with repeated runs of {\sc ChosenPath}}
  \label{fig:repeat}
\end{figure}

Recall can be boosted to any desired level by performing multiple iterations of {\sc ChosenPath}.
Each {\sc ChosenPath} iteration finds points independently and by accumulating the points found over several runs any desired recall can be reached. Of course this also means the cost of achieving a given recall is exponentially growing with the recall.

Figure Speed 1 and Speed 1 depict speedups over {\sc All} for $50\%$ and $90\%$ recall respectively.



\subsubsection{Concurrency}
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.4\textwidth]{parallel.pdf}
  \caption{Parallel runs on Netflix dataset}
    \label{fig:parallel}
\end{figure}
The \cpsj is very simple to run in parallel. It requires only a different random seed for each instance and merging and deduplication of the final results.
We have conducted some preliminary experiments by simply starting the process on separate threads.
The results show that it takes around $1.5$ times longer to run the \cpsj $4$ times on $4$ threads, than to run it once on one thread (see example Figure\ref{fig:parallel}).
Without any modifications, \cpsj can exploit any number of cores, only limited by read access to the input data and collection and deduplication of the output.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "simfilter"
%%% End:


